NESTFUL: A Benchmark for Evaluating LLMs on Nested Sequences of API Calls

The resurgence of autonomous agents built using large language models (LLMs) to solve complex real-world tasks has brought increased focus on LLMs' fundamental ability of tool or function calling. At the core of these agents, an LLM must plan, execute, and respond using external tools, APIs, and custom functions. Research on tool calling has gathered momentum, but evaluation benchmarks and datasets representing the complexity of the tasks have lagged behind. In this work, we focus on one such complexity, nested sequencing, with the goal of extending existing benchmarks and evaluation. Specifically, we present NESTFUL, a benchmark to evaluate LLMs on nested sequences of API calls, i.e., sequences where the output of one API call is passed as input to a subsequent call. NESTFUL contains 1800+ nested sequences where all the function calls are executable. Experimental results on a variety of models show that the best-performing model (GPT-4o) achieves a full sequence match accuracy of 28% and a win-rate of 60%, necessitating a large scope for improvement in the nested sequencing aspect of function calling. Our analysis of these results provides possible future research directions for the community, in addition to a benchmark to track progress. We have released the NESTFUL dataset under the Apache 2.0 license at https://github.com/IBM/NESTFUL.

==> sections/authors.tex <==
\vspace{-2cm}
\begin{center}
\textbf{Kinjal~Basu}$^1$$^,$$^\ddagger$\quad
\textbf{Ibrahim~Abdelaziz}$^1$$^,$$^\ddagger$\quad
\textbf{Kelsey Bradford}$^2$\quad
\textbf{Maxwell~Crouse}$^1$\quad
\textbf{Kiran Kate}$^1$\quad
\textbf{Sadhana~Kumaravel}$^1$\quad
\textbf{Saurabh Goyal}$^1$\quad
\textbf{Asim Munawar}$^1$\quad
\textbf{Yara Rizk}$^1$\quad
\textbf{Xin Wang}$^1$\quad
\textbf{Luis~Lastras}$^1$\quad
\textbf{Pavan~Kapanipathi}$^1$$^,$$^\ddagger$\quad

$^1$IBM Research, $^2$Georgia Institute of Technology \\
\vspace{0.2cm}
% $^\star$Equal Contribution \\
$^\ddagger$Corresponding Authors \\
\texttt{\{kinjal.basu, ibrahim.abdelaziz1\}@ibm.com, kapanipa@us.ibm.com}

\end{center}


==> sections/data_schema.tex <==
\section{\dataset{} Dataset Schema} \label{sec:data_schema}

Each data instance in the \dataset{} dataset consists of a question-answer pair, where the answer is a sequence of API calls represented as a list of JSON objects. Each JSON object corresponds to an API, including its `name' and `arguments'. Additionally, a unique variable name is assigned to each JSON object under the key `label', which distinctly identifies each API, even when two identical APIs with different arguments appear in the same sequence (parallel API calls). Argument values that need to be grounded with results from previous function calls are enclosed in a \$ sign and formatted as \texttt{\$\{variable\_name\}.\{parameter\}\$}, where \texttt{\{variable\_name\}} refers to the API whose results will be used, and \texttt{\{parameter\}} specifies the output parameter of that API response. Below is the template for the data schema:

\smallskip
\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
  "input": <User Query>,
  "output": [
    {
      "name": <API Name>,
      "arguments": {
        <arg_1>: <value from user query>,
        <arg_2>: <value from user query>,
        ...
      },
      "label": <variable_name>
    },
    {
      "name": <API Name>,
        "arguments": {
          <arg_1>: <value from user query>,
          <arg_2>: ${variable_name}.{parameter}$,
          <arg_3>: <value from user query>,
          ...
        },
        "label":  <variable_name>
    }
    ...
  ]
}
\end{lstlisting}
\end{nolinenumbers}
\smallskip




==> sections/dataset_collection_original.tex <==
\section{Dataset Collection}
\label{sec:dataset}
% \begin{figure}[t!]
% \begin{center}
% \includegraphics[width=\columnwidth]{AnonymousSubmission/LaTeX/figures/nestful_dataflow.drawio.pdf}
% \caption{Execution of Nested Sequence of API data}
% \label{fig:data_flow}
% \end{center}
% \end{figure}





\dataset{} dataset comprises of more than 1,800 instances designed for benchmarking tool-augmented large language models, with a focus on nested sequencing. Each instance consists of 1) a user query, 2) a list of available tools to answer the given query, 3) the final answer that should be obtained once the tools are executed. We also provide the corresponding Python codes for every API in the library as well as a mechanism to run the input query via any LLM, execute the tools predicted by the LLM, and provide the final answer.

\dataset{}'s data comes from two domains; 1) math-based data and 2) generic functions for everyday use. We describe below the process followed to create each data category. 

\subsection{Math and Reasoning Data}
For the first part of \dataset{}, we relied on datasets that test the model for nested function calling in the math domain. In particular, we build on MathQA~\cite{mathqa}; a benchmark designed for evaluating the ability of AI models to solve mathematical word problems. It consists of questions that test numerical reasoning and problem-solving skills, requiring models to both understand the text of a word problem and perform mathematical operations to arrive at the correct solution. An example is shown here:

\smallskip
\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
  "Problem": "An artist wishes to paint a circular region on a square poster that is 3.4 feet on a side. if the area of the circular region is to be 1/2 the area of the poster, what must be the radius of the circular region in feet?",
  "Operation Stack": "square_area(3.4) divide(#0,1/2) divide(#1,const_pi) sqrt(#2)",
  "Answer":  1.3543
}
\end{lstlisting}
\end{nolinenumbers}
\smallskip

The \textit{Operation Stack} provides the following ordered sequence of tools to call: 1) ``square\_area(3.4)`` $\rightarrow$ 11.56, 2) ``divide(11.56, 1/2)`` $\rightarrow$ 5.78, 3) ``divide(5.78, const\_pi)`` $\rightarrow$ 1.8343, and finally 4) ``sqrt(1.8343)`` $\rightarrow$ 1.3543. 

To create \dataset{}, we did the following steps:
\begin{itemize}
    \item \textbf{API/Tool specifications}: we created specifications for all the tools in MathQA dataset. This covers 40 tools in total; e.g.  divide, remainder, volume\_cylinder, permutation ... etc. For each tool, we define the name, description, and a detailed description of the tool input and output parameters. An example of such specification is shown below:

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
        "name": "surface_sphere",
        "description": "Calculate the surface area of a sphere",
        "parameters": {
            "arg_0": {
                "description": "Radius of the sphere",
                "type": "float"
            }
        },
        "output_parameter": {
            "result": {
                "description": "Surface area of the sphere",
                "type": "float"
            }
        }
    }
\end{lstlisting}
\end{nolinenumbers}

    \item \textbf{Tool calling input-output pairs}: To build the test instances, we used the test set of MathQA where we used the "problem" definition as our query and parsed the "annotated formula" into a nested sequence of tool calls. For the example above, we generate the following pair:
    
\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
  "input": "An artist wishes to paint a circular region on a square poster that is 3.4 feet on a side. if the area of the circular region is to be 1/2 the area of the poster, what must be the radius of the circular region in feet?",
  "tools": "[{"name": "square_area", "arguments": {arg_0: 3.4}, "label": "var_0"},  {"name": "divide", "arguments": {arg_0: $var_0.result$, arg_1: 0.5}, "label": "var_1"}, {"name": "divide", "arguments": {arg_0: $var_1.result$, arg_1: pi}, "label": "var_2"}, {"name": "sqrt", "arguments": {arg_0: $var_2.result$}, "label": "var_3"}]",
  "answer":  1.3543
}

\end{lstlisting}
\end{nolinenumbers}    

        \item \textbf{Executable Code and Filtering:} For each tool, we also generate its corresponding implementation in Python. With this, we can also execute the nested call sequence and match the execution result with the gold answer. This ensures that correctness of the set of corresponding tools and the code execution too. We then filter out any sample where we can not reproduce the gold answer from executing the nested tool calls. 
\end{itemize}

This process resulted in 1,415 test samples covering 40 tools with an average XX tool calls per sample. {\color{red} ADD MORE STATS}

\subsection{Generic Tools}
We also curated test examples based on generic tools from StarCoder2-Instruct dataset\footnote{\url{https://huggingface.co/datasets/bigcode/self-oss-instruct-sc2-exec-filter-50k}}. This dataset has a total of 50K functions defined in Python and cover a wide range of tools that can be used. To created nested tool calling test set from this dataset, we followed the following steps:

\begin{itemize}
    \item \textbf{Creating Specifications}: StarCoder2-Instruct has Python implementations with docstrings that can be used to create API specifications. We show an example below:

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
def angle_rotation(arr, k):
    """Rotates the elements in the array by `k` positions in the right direction.
    Args:
        arr: The array of numbers.
        k: The number of positions to rotate the elements in the array.
    Returns:
        The array after rotating the elements by `k` positions in the right direction.
    """
    if len(arr) < k:
        k = k % len(arr)
    return arr[len(arr)-k:] + arr[:len(arr)-k]
\end{lstlisting}
\end{nolinenumbers}  
 For each Python function, we 1) use an LLM (Mixtral 8x22B\footnote{\url{https://huggingface.co/mistralai/Mixtral-8x22B-Instruct-v0.1}}) to generate the possible Python types of the input and output arguments, and then 2) we validate and execute the function code itself to ensure it does not produce any errors. Once both steps are done, we generate a corresponding JSON specification for each function documenting its input/output arguments. For the above function, this results in:
\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
        "name": "angle_rotation",
        "description": "Rotates the elements in the array by `k` positions in the right direction.",
        "output_parameters": {
            "properties": {
                "output_0": {
                    "description": "The array after rotating the elements by `k` positions in the right direction.",
                    "type": "array"
                }
            }
        },
        "parameters": {
            "properties": {
                "arr": {
                    "description": "The array of numbers.",
                    "items": {
                        "type": "integer"
                    },
                    "type": "array"
                },
                "k": {
                    "description": "The number of positions to rotate the elements in the array.",
                    "type": "integer"
                }
            },
            "required": [
                "arr",
                "k"
            ],
            "type": "object"
        }
    }
\end{lstlisting}
\end{nolinenumbers}  

\item \textbf{Tool calling input-output pairs}: To create input-output instance, we synthetically generated 446 nested tool calling instances. To do so, we leveraged DiGiT\footnote{\url{https://github.com/foundation-model-stack/fms-dgt}} synthetic data generation framework where we curated manually 10 seed examples and used Mixtral-8x22B as the teacher model to generate the rest. We also built a validator to check the correctness of the produced samples w.r.t. ensuring the tools/parameters used are not hallucinated, required parameters are specified and there is at least one nested tool call in the output sequence. 

\item \textbf{Filtering:} We further filter the generated input/output pairs by executing their gold nested sequence of API calls to ensure it works and attach the result as the gold answer. For function that has a randomness element; e.g. generating a random list, we set a fixed seed for all our experiments. {\color{red}Other filtering approaches??}

\end{itemize}

From this category of data, we generated 446 test examples covering more than 4,400 different tools. {\color{red}ADD MORE STATS}

% \subsection{Executable APIs} \label{sec:exec_apis}
% The executable portion of the \dataset{} dataset is curated using APIs sourced from RapidAPI. We manually gather 39 different APIs across various domains, including flight booking, Instagram information, restaurant and hotel searches, music, finance, and more. For each API, we collect essential specifications such as API names, query/path parameters, output parameters, host, endpoint, etc. We also write descriptions by hand for all parameters (query, path, and output). Following is a template of the specification.

% \smallskip
% \begin{nolinenumbers}
% \begin{lstlisting}[language=json,firstnumber=1]
% {
%   "name": <API name>,
%   "description": <API description>,
%   "method": <API methods, such as GET, POST, ...>,
%   "endpoint": <API endpoint path>,
%   "host": <API host path>,
%   "url": <API URL from RapidAPI for reference>,
%   "query_parameters": <dictionary of query parameters (if any)> with parameter name, description, type, required field (boolean)>,
%   "path_parameters": <dictionary of path parameters (if any)> with parameter name, description, type, required field (boolean)>,
%   "output_parser": <location of the output parameters in the API response object>,
%   "output_parameters": <the parameters in the API response>
% }


% \end{lstlisting}
% \end{nolinenumbers}
% \smallskip

% Next, based on the gathered API specifications, we construct the executable dataset as a collection of query-answer pairs, where the answers consist of sequences of executable APIs. Our code processes the outputs, calling each API sequentially to achieve the final result. The questions are human-annotated, ensuring that the final answer can only be obtained by executing the APIs in a nested manner—where the output of one API is used as the input for the subsequent API. An example is provided below:

% \smallskip
% \begin{nolinenumbers}
% \begin{lstlisting}[language=json,firstnumber=1]
% {
%     "input": "What is the time difference between Morocco and New York?",
%     "output": [
%       {
%         "name": "WeatherAPI.com_Time_Zone_API",
%         "arguments": {
%           "q": "Morocco"
%         },
%         "label": "var1"
%       },
%       {
%         "name": "WeatherAPI.com_Time_Zone_API",
%         "arguments": {
%           "q": "New York"
%         },
%         "label": "var2"
%       },
%       {
%         "name": "CipherCircuit_Math_Assistant
%                   _CalculateAllArithmeticOperations",
%         "arguments": {
%           "numbers": "$var1.localtime$ - $var2.localtime$"
%         },
%         "label": "var3"
%       },
%       {
%         "name": "var_result",
%         "arguments": {
%           "time_difference": "$var3.result$"
%         }
%       }
%     ]
% }
% \end{lstlisting}
% \end{nolinenumbers}
% \smallskip

% \subsection{Non-Executable APIs}
% For non-executable data curation, we begin by collecting API specifications from the Glaive\footnote{\url{https://huggingface.co/datasets/glaiveai/glaive-function-calling-v2}} and Schema Guided Dialog (SGD)\footnote{\url{https://github.com/google-research-datasets/dstc8-schema-guided-dialogue}} datasets. SGD dataset has a limited set of APIs, but it has full specifications, including input and output parameters. On the other hand, Glaive APIs do not have output parameters, for which, we created the output parameters manually. 

% We then used DiGiT synthetic data generation framework\footnote{https://github.com/foundation-model-stack/fms-dgt} to systematically create a set of nested sequence data. This involves using seed examples along with detailed instructions to prompt the Mixtral-8x22b-Instruct model\footnote{\url{https://huggingface.co/mistralai/Mixtral-8x22B-Instruct-v0.1}}. Finally, we perform a two-step filtration process to refine the dataset. First, we programmatically validate the samples to check for hallucinations and ensure that the output APIs adhere to the specifications; required parameters are specified and output parameters are correct. Then, we manually review and exclude any examples with semantic errors, incorrect API sequence order, or improper variable assignments. Below is an example based on Glaive API list:

% \smallskip
% \begin{nolinenumbers}
% \begin{lstlisting}[language=json,firstnumber=1]
% {
%     "input": "Encrypt the email address 'john.doe@gmail.com' with the key 'abc123' and then add a new contact with the encrypted email, name 'John Doe', and phone '123-456-7890'",
%     "output": [
%         {
%             "name": "encrypt_data",
%             "arguments": {
%                 "data": "john.doe@gmail.com",
%                 "encryption_key": "abc123"
%             },
%             "label": "var1"
%         },
%         {
%             "name": "add_contact",
%             "arguments": {
%                 "email": "$var1.encrypted_data$",
%                 "name": "John Doe",
%                 "phone": "123-456-7890"
%             },
%             "label": "var2"
%         }
%     ]
% }
% \end{lstlisting}
% \end{nolinenumbers}
% \smallskip

